Gradient-based Editing of Memory Examples for Online Task-free Continual Learning

We explore task-free continual learning (CL), in which a model is trained to avoid catastrophic forgetting in the absence of explicit task boundaries or identities. Among many efforts on task-free CL, a notable family of approaches are memory-based that store and replay a subset of training examples. However, the utility of stored seen examples may diminish over time since CL models are continually updated. Here, we propose Gradient based Memory EDiting (GMED), a framework for editing stored examples in continuous input space via gradient updates, in order to create more "challenging" examples for replay. GMED-edited examples remain similar to their unedited forms, but can yield increased loss in the upcoming model updates, thereby making the future replays more effective in overcoming catastrophic forgetting. By construction, GMED can be seamlessly applied in conjunction with other memory-based CL algorithms to bring further improvement. Experiments validate the effectiveness of GMED, and our best method significantly outperforms baselines and previous state-of-the-art on five out of six datasets. Code can be found at https://github.com/INK-USC/GMED.

==> chaps/background.tex <==
\section{Problem Formulation}
\label{sec:background}
\vspace{-0.1cm}

% In this section we first revisit the problem formulation of task-free continual learning and then introduce  memory-based continual learning methods.
%\arka{Section 3 Preliminaries can be merged with Section 4, 3.1 3.2 can be merged into one subsection.}

\input{floats/overview_fig}

% \vspace{-0.1cm}
% \subsection{Problem formulation}
% \label{ssec:problem_formulation}
% We suppose the model visits an online non-stationary stream of data instances.

We first describe the problem formulation of the task-free continual learning setting, followed by details on current memory-based approaches and their limitations.

\textbf{Mathematical Formulation.} 
In task-free continual learning, we consider a (potentially infinite) stream of data examples $D$, having a non-stationary data distribution, \ie, the data distribution $p(x,y)$ evolves over time.
% (\textit{i.e.}, non i.i.d distribution).
% At each time step $t$, the model receives a single or a mini batch of labeled examples $(x_t, y_t)$ from the data stream $D$. 
Let $(x_t, y_t)$ denote the labeled example (or mini-batch of examples) received by the model at time-step $t$ from the data-stream $D$.
% For simplicity, here 
We assume (for simplicity) that $(x_t, y_t)$ is generated by first sampling a \textit{latent} ``task" $z \sim p(z; t)$, followed by sampling a data example from a joint data distribution $p(x, y|z)$ that is conditioned on task $z$, \textit{i.e.}, $(x_t, y_t) \sim p(x, y|z)$. 
Here $p(z; t)$ is non-i.i.d and time-dependent. 
We assume the latent task $z$ is not revealed to the model at training or testing. 
We emphasize that the online learning setup prohibits learning a task for multiple epochs until convergence before proceeding to the next task.
%\arka{Both $P(z; t), P(x,y|z;t)$ are non-i.i.d and time-dependent.}
%\arka{Is the above assumption used in prior work also? If so should be mentioned}

Using the above definitions, 
% task-free online continual learning seeks a classification model 
we denote a classification model learning in task-free online continual setting as
% $f(x;\theta)$, parameterized by $\theta$, over new example(s) $(x, y)$ from the data stream $D$ that minimizes a predefined loss $\ell(x, y; \theta)$ while not increasing the loss on previously seen examples. 
$f(x;\theta)$, parameterized by $\theta$, which given new example(s) $(x, y)$ from the data stream $D$  minimizes a predefined loss $\ell(x, y; \theta)$ while not increasing the loss on previously seen examples. 
Specifically, if $p_c(x,y;t)$ is the cumulative data distribution visited until a time step $t$, our goal is to minimize the expected loss $\E_{p_c(x,y;t)} \ell(x,y; \theta)$ (or similarly maximizing metrics such as accuracy) evaluated over the model at the end of the training.
Essentially, the objective implies retaining performance on previous tasks is crucial. 
% \arka{need in-line math eqn}
%which consists of new examples that follows the distribution of the stream $D$. %  The model is trained over a single pass of the stream. We evaluate the model performance on a test set which follows the data distribution the model has visited since the beginning of the training.

% \subsection{Memory-based CL Methods}
\smallskip
\noindent
% \textbf{Limitations of Memory-based CL Methods.}
%\xiang{compress a bit and focus on presenting the holes in previous methods.]}

\textbf{Memory-based CL algorithms} (\eg, Experience Replay (ER)~\citep{Robins1995CatastrophicFR}) store a subset of previously seen examples in a fix-sized replay memory $M$. 
At each training time step $t$, the algorithm chooses one or a mini-batch of memory examples (denoted by $(x_m, y_m)$) for replay. 
In the online task-free scenario, the memory can be populated with online strategies such as reservoir sampling~\citep{Vitter1985RandomSW}.

\xiang{Note: can we frame this part in a more systematic way, like in Fig. 1, so people get a better sense of the moving parts and distinctions for this family of methods.}

\textbf{Limitations} While a number of recent works improve memory based CL algorithms with more fine-grained strategies to select examples, these methods are inherently limited by storing original examples, which does not guarantee to find the most ``useful'' examples in the current context. 
Moving apart from replaying real examples, a line of works on deep generative replay~\citep{Shin2017ContinualLW, Hu2019OvercomingCF, Rostami2019ComplementaryLF} generates synthetic examples to replay with a generative model trained online, but the approach is rather an alternative to draw past examples in a restricted scenario.
~\citet{Buzzega2020RethinkingER} show independent data augmentations over drawn examples to replay significantly improve the performance, but the augmentation is less principled.
~\citet{Chaudhry2020UsingHT} learn one synthetic examples per class per task that suffers most from the forgetting, but the method only operates in the task-aware scenario. 
\arka{Is there only one limitation?}

==> chaps/method_old.tex <==
\section{Method}
The model visits a non-stationary distribution of stream examples and receive a mini batch of stream examples $D_t$ at each time step. We write the data distribution at current time step $t$ as $P(D_t)$, and write $P(D_{1:t})$ for the data distribution seen so far until time step $t$. We suppose $P(D_{1:t})$ is a mixture of multiple components, and each example $x$ is generated by sampling from one component $z$. In prior works, a component usually specifies a ``task''. If we employ reservoir sampling, the examples stored in memory $\mathcal{M}$ exactly follow the distribution $P(D_{1:t})$.  
Informally, the goal of memory scheduling or editing is to search for a subset of examples from $D$ so that when the training ends the overall metric scores (accuracy etc.) is maximized. However, deciding how to store or edit is an difficult online decision problem without hindsight, as we assume no idea about future data distribution. Thus, we introduce our first assumption about "high-quality" examples that are advantageous for alleviating forgetting and improving overall performance which should be kept in the memory.

\textbf{Assumption 1}. Training the model with the most interfering example from a task $z$ will best maintain the performance on all the examples from the task $z$ when the training ends. The interference (or forgetting) is defined as the training loss increase at the end of training compared to when the example is initially used for training the model. The objective of the memory optimization is therefore $\textrm{argmax}\ L(x; \theta_T) - L(x; \theta_t)$, where $\theta_t$ and $\theta_T$ are model parameters at time step $t$ and when the training ends.

However, determining the most interfering examples also requires hindsight and is not possible during training. We therefore estimate the interference of examples with the loss increase when the model is trained on a mini-batch of examples from the stream. 

Next, our second assumption is about the ``coverage'' of examples stored in the memory. Apparently, storing only interfering examples for a single task will hurt performance on other tasks. If $\mathcal{M}$ consists of random samples drawn from the data visited so far (e.g. by reservoir sampling), the coverage is ensured. However, since we are about to perform editing on memory examples, the coverage is no longer guaranteed. Given an edited memory $\mathcal{M}^\prime$, we need to explicitly quantify how likely the examples in the memory are randomly drawn from $P(D_{1:t})$. Formally, it is to keep the posterior probability $P(\Theta_D | \mathcal{M}^\prime )$ high given the observations $\mathcal{M}^\prime$, where $\Theta_D$ is the parameters of the distribution $P(D_{1:t})$. Unfortunately, since $\Theta_D$ is unknown to us, it is difficult to determine whether the modified memory $\mathcal{M}^\prime$ are likely to be drawn randomly. We therefore carry out our second assumption.

\textbf{Assumption 2}. The coverage of examples are maintained after any memory editing by our algorithm. Formally, $P(\Theta_D | \mathcal{M}^\prime )$ is almost as high as $P(\Theta_D | \mathcal{M})$.

We finally add an optimization constraint that training on edited examples from $\phi$ should not cause degraded model performance on the data seen so far, i.e., $D_{1:t}$. To implement this constraint, we randomly sample another mini-batch of memory examples $\phi_v$ from current memory. Recall that if we assume no memory editing then $\phi_v$ is a random set of samples drawn from $D_{1:t}$. Therefore, we can approximately measure how the edited examples interfere with overall data by measuring its interference between the edited exampls from $\phi$ (noted as $\phi^\prime$) and $\phi_v$. To prevent the interference, we train the model on $\phi_v$ and reject memory editing if the edited examples have higher loss compared to that before editing. Note that we can also measure loss change on $\phi_v$ before and after we train on for each of the memory example, but this implementation is much more time consuming.

In short, our algorithm edits memory so that they are more interfering with current stream examples, and meanwhile prevents the interference with a random subset of memory examples. It tries to make memory examples more likely to interfere with future data while not interfere with past data.

(I actually find this added constraint a bit strange after write it down)

==> chaps/setting_old.tex <==
\section{Problem Formulation}
\subsection{Learning Objective}
The learning objective of our model is to perform language modeling with visual inputs. The training data consists of image input $x_{img}$, bounding boxes $x_{bbox}$, and the textual input $x_{text}$. Similar to the settings in~\cite{surs2019learning}, the bounding boxes are \emph{not} associated with ground truth object categories contained in the box. The model should learn to associate each bounding box with text input. During inference, the model is required to predict a masked word in the text. The masked words are either nouns, adjectives, or verbs. 

\subsection{Testbed}
We use the MS COCO~\cite{lin2014microsoft} dataset to construct a data stream. In COCO dataset, each image is associated with several captions and several bounding boxes annotated with object classes (such as \textit{people}, \textit{sport balls}). These object names do not necessarily appear in the caption text in their canonical form, but are likely to appear in various surface forms (such as \textit{woman}, \textit{football}). 
% We construct the data stream so that the object class roughly comes one by one as a ``task''. Formally, a task is a distribution of data conditioned on the object class $c_i$.
% \begin{equation}
%     \mathcal{T}_i = p(x_{img}, x_{bbox}, x_{text} | c_i).
% \end{equation}
% where $c_i$ is also called the task identifier of the task $\mathcal{T}_i$. The task identifier is never exposed to the model at training or at inference. Besides, to make the setting more realistic, there is a small chance that previous objects appear later in the stream, and the new task is introduced continuously until replacing the current task.
We construct the data stream so that the underlying object classes follow a non-stationary distribution. Formally, training instances are drawn from a distribution conditioned on the object class $c$, which itself follows a categorical distribution which varies over time.

\begin{equation}
\begin{split}
     c &\sim Cat(\pi(t)) \\
     x_{img}, x_{bbox}, x_{text} &\sim P(x_{img}, x_{bbox}, x_{text} | c)
     \end{split}
\end{equation} 

The parameter $\pi(t)$ depends on the time step $t$, making the object distribution non-stationary. At the most extreme case, the object class comes one by one with clear boundaries, known as ``different tasks'' in prior continual learning literature. However, we will experiment with a more realistic scenario, where there are repetitions of old classes. We also experiment with the case where the parameters $\pi(t)$ changes gradually and slowly over time, so that there are no clear boundaries. Note that inferring task identity in this scenario is not trivial. On one hand, the underlying data stream does not have clear task boundaries. On the other hand, because of the variation of the surface forms of objects, it is difficult to determine the underlying object class of current data. 


\subsubsection{More datasets}
We will also experiment with other image captioning dataset, such as Flickr30k~\cite{Plummer2015Flickr30kEC}, which is a crowd-sourced image captioning dataset collected in a similar way as MSCOCO; Conceptual Captions~\cite{sharma-etal-2018-conceptual}, which is a large scale automatically created image captioning dataset. 

\begin{table*}[!]
\small
\centering
\begin{tabular}{c|c|c|c|c|c}
\hline
\textbf{}                             & \textbf{}                       & \textbf{Task-aware} & \multicolumn{3}{c}{\textbf{Task-free}}                                                     \\ \hline
\textbf{}                             & \textbf{}                       & \textbf{Given Boundaries}           & \textbf{Sudden task switch} & \textbf{Continuous task drift} & \textbf{Revisit of old tasks} \\ \hline
\multirow{2}{*}{\textbf{Data based}}  & Replay buffer                   & T                   & T?                           & T?                              & T?                            \\ 
                                      & Distillation, DGR & T                   & F                           & F                              & F                            \\ \hline
\multirow{4}{*}{\textbf{Model based}} & Task-aware Reg.                  & T                   & F                           & F                              & F                            \\ \ 
                                      & Task-free MAS                   & T                   & T                           & F                              & F                         \\ 
                                      & Bayesian                        & T                   & T                           & T                              & T?  \\ 
& Task inference & T & T & T & T
                                      \\ \hline
\end{tabular}
\caption{Compatibility of continual learning algorithms and different continual learning scenarios. Among them, \textbf{Task-free MAS}~\cite{aljundi2019task}, \textbf{Bayesian}~\cite{Zeno2018TaskAC}, and \textbf{Task-inference} based approaches~\cite{He2019TaskAC, Rao2019ContinualUR, Nagabandi2018DeepOL} are specifically proposed for task-free scenarios. Here, \textbf{task-aware reg.} based approaches include EWC, SI, MAS, Hypernets and etc. T indicates the compatibility is verified by experiments; T? indicates plausible compatibility; F indicates the algorithm is not easily compatible with the scenario. }
\label{tab:challenge}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{l|l|l}\hline
                  & \textbf{Prior works}  & \textbf{Ours}                            \\ \hline
Data distribution & Clear task boundaries & + Blur task boundaries or continuous drift \\ \hline
Backend task      & Classification        & Language modeling                        \\ \hline
Goal    & Alleviating catastrophic forgetting       & + Fast learning on novel concepts \\ \hline
\end{tabular}
\caption{Difference of settings between our works and majority of prior continual learning literature.}
\end{table*}

\subsection{Evaluation}
\textbf{Novel instances} To evaluate the prediction performance of the model on new instances, we may plot the accuracy curves on a held out validation set and test set which consists of all classes visited so far alongside training. 

\textbf{Novel classes} We also evaluate how fast the model learns a new object by plotting the predicting accuracy just for the object after it is introduced in the stream. After obtaining the curves, we compare the curves quantitatively with area under the curve and the value of the curve at the end.

% \subsection{Intuition of the Formulation and Potential Data Resources}
% \textbf{Intuition}. The learning objective and the data distribution is inspired by how babies learn language from visual data. The input to the model is based on the assumption that the babies are born with intelligence to segment visual objects and only need to learn how to associate visual objects to language. The language modeling objective of our model resembles the language acquisition of babies. The non-stationary and streaming training data with inherent repetitions of old tasks mimics the environments where the babies learn from. 

% \textbf{Potential Data Resources}. In addition the COCO dataset, we are considering to incorporate datasets which provide more realistic environments. Prior works incorporate TV series and videos as more realistic datasets for studying continual learning~\cite{aljundi2019task} or mimicking baby learning~\cite{surs2019learning}, but not both at the same time. There are resources for studying visually grounded word acquisition of babies built upon synthetic 3D objects~\cite{stojanov2019incremental} and even real scenes~\cite{bambach2018toddler}, but their visual input is only associated with an object category instead of a natural language input. Our formulation is more similar to how children learn from both visual input and natural language, for example, from reading cartoon books or cartoon videos, but we could not find existing resources for these.


==> floats/ablation.tex <==
\begin{table*}
\centering
\scalebox{0.72}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Methods / Datasets} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Permuted\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rotated\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ CIFAR-10\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ CIFAR-100\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ mini-ImageNet\end{tabular}} \\ \midrule
\textbf{ER + GMED}          & 82.68 $\pm$ 2.1                                                & 79.70 $\pm$ 1.1                                                   & 77.89 $\pm$ 0.9                                                  & 35.01 $\pm$ 1.5                       &    20.87 $\pm$ 1.4                        & 27.79 $\pm$ 0.7                                                        \\
\textbf{ER + Random Edit}   & 81.04 $\pm$ 2.1                                                & 78.99 $\pm$ 0.5                                                   & 77.59 $\pm$ 1.0                                                  & 32.26 $\pm$ 1.9                        &         20.73 $\pm$ 1.1                  & 26.23 $\pm$ 2.1                                                        \\                                        \midrule
\textbf{MIR + GMED}         & 87.86 $\pm$ 1.1                                                & 80.11 $\pm$ 1.2                                                   & 79.16 $\pm$ 0.9                                                  & 35.54 $\pm$ 1.9                         &      21.49 $\pm$ 0.6                    & 26.29 $\pm$ 1.2                                                        \\
\textbf{MIR + Random Edit}  & 84.76 $\pm$ 1.4                                                & 79.76 $\pm$ 0.6                                                   & 78.19 $\pm$ 1.0                                                  & 35.39 $\pm$ 3.0                          &     19.77 $\pm$ 1.1                    & 24.86 $\pm$ 0.7                                                        \\ \bottomrule



\end{tabular}
}
\caption{Performance when we updates memory examples to a random direction (Random Edit), compared to ER+GMED and MIR+GMED.}
\label{tab:ablation}
\vspace{-0.1cm}
\end{table*}

%\midrule
% \textbf{ER + Random Edit} & $80.13 \pm 2.9$ & $78.85 \pm 0.2$ & $76.40 \pm 1.7$ & $34.72 \pm 1.6$ & $25.73 \pm 2.0$ \\
% \textbf{ER + Hindsight Edit} & $70.32 \pm 3.9$ & $79.23 \pm 0.6$ & $76.33 \pm 1.1$ & $33.08 \pm 3.3$ & $27.27 \pm 1.7$ \\

==> floats/checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
     \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
 


%\begin{table*}[t]
% \centering
% \caption{NeurIPS 2021 submission checklist.
% }
% \scalebox{0.7}{
% \begin{tabular}{ p{13cm}p{5cm} }
% \toprule
% Question &  Response \\ \midrule
% \rowcolor{na} 1. For all authors & Applicable \\
% (a) Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope & Yes \\
% (b) Have you read the ethics review guidelines and ensured that your paper conforms to them? & Yes \\
% (c) Did you discuss any potential negative societal impacts of your work? & N/A  \\
% (d) Did you describe the limitations of your work? & Yes \\

% \rowcolor{na} 2. If you are including theoretical results... & Not Applicable \\
% % (a) Did you state the full set of assumptions of all theoretical results? & Yes \\
% % (b) Did you include complete proofs of all theoretical results & N/A \\
% \rowcolor{na} 3. If you ran experiments... & Applicable \\
% (a) Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? & Yes \\
% (b) Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? & Yes \\
% (c) Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? & Yes \\
% (d) Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? & Yes \\
% \rowcolor{na} 4. If you are using existing assets (e.g., code, data, models) or curating/releasing new assets... & Applicable \\
% (a) If your work uses existing assets, did you cite the creators? & Yes \\
% (b) Did you mention the license of the assets? & No \\
% (c) Did you include any new assets either in the supplemental material or as a URL? & N/A (we have not introduced new assets in the paper) \\
% (d) Did you discuss whether and how consent was obtained from people whose data you're using/curating? & No \\
% (e) Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? & Yes (it does not contain such information) \\
% \rowcolor{na} 5. If you used crowdsourcing or conducted research with human subjects & Not Applicable \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

==> floats/compare_mem_aug.tex <==
% \begin{table*}[]
%     \centering
%     \begin{tabular}{c|c}
%         \textbf{ER$_{aug}$}   & 79.91 $\pm$ 1.7                                                &                                                 & 80.60 $\pm$ 1.3                                      & 46.61 $\pm$ 2.0                       &         20.73 $\pm$ 1.1                  &  31.36 $\pm$ 2.1                                                        \\ 
%         \textbf{ER$_{aug}$ + GMED}   & 82.39 $\pm$ 2.1                                                &                                                   & 80.66 $\pm$ 1.2                                                 &   46.50 $\pm$ 2.4                  &         20.73 $\pm$ 1.1                  & 32.45 $\pm$ 1.2                  
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}

% \begin{table*}
% \centering
% \scalebox{0.72}{
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \textbf{Methods / Datasets} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Permuted\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rotated\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ CIFAR-10\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ CIFAR-100\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ mini-ImageNet\end{tabular}} \\ \midrule
%                                                   \\ 
%         \; + GMED   & 82.39 $\pm$ 2.1                                                &                                                   & 80.66 $\pm$ 1.2                                                 &   48.34 $\pm$ 2.6                  &         14.46 $\pm$ 1.3                  & 32.45 $\pm$ 1.2            \\   \bottomrule 
%     \end{tabular}
% }
% \caption{Performance when we updates memory examples to a random direction (Random Edit), compared to ER+GMED and MIR+GMED.}
% \label{tab:ablation}
% \vspace{-0.1cm}
% \end{table*}

==> floats/comple_fig.tex <==
\begin{figure}[tb]
\vspace{-0.2cm}
    \centering
    \includegraphics[width=0.98\linewidth]{figs/new_fig1_2.pdf}
    \vspace{-0.2cm}
    \caption{
    \textbf{\arka{Figure can made more compact. Can also add comparison to GEN-MIR, highlighting the main points of difference.} Overview of key components in memory-based continual learning approaches.} Prior works study (a) memory population and (b) memory sampling strategies, improving how to store streaming examples into the memory or sampling them from memory for replay. In contrast, our work focuses on ``editing'' memory examples which can subsequently be stored, edited again, and be replayed.
    % to search input-label pairs to replay in the continuous input space. 
    %\bill{Is this figure referred in the paper anywhere? I think it may be helpful to be used for connecting the natural-langueg arguments in the text to a better visualized explantion. }
    }
    %\xiang{can we fit in generative replay methods?}
    \label{fig:compare} 
    \vspace{-0.4cm}
\end{figure}


    %Categorization of memory-based methods on Task-free Continual Learning. Reservoir sampling and Sampling from Memory are the ways that Experience Replay (ER) uses to construct and replay memory respectively. In the recent line of works, Gradient based Sample Selection (GSS) and Hindsight Anchor Learning (HAL) explored ways to construct memory, while Maximally Interfering Retrieval (MIR) focused on replay strategy. Our method, Gradient-based Memory Editing (GMED) falls under the former category but provides a new angle to memory construction. \xiang{can revisit.}


==> floats/edit_viz.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
    \centering
    \includegraphics[width=0.48\textwidth]{figs/edit_viz.pdf}
    \vspace{-0.3cm}
    \caption{Visualization of the editing on examples from first two tasks in the Split MNIST dataset. The first and the second row shows original and the edited examples, while the third row shows the difference between the edited examples and the original ones.}
    \label{fig:edit_viz}
\end{wrapfigure}


==> floats/legacy_main_tab.tex <==
\begin{table*}[tb]

\caption{\small \textbf{Mean and standard deviation of final accuracy (\%)} in 10 runs for non-model-expansion-based approaches. See Table~\ref{tab:comp_cndpm} for the results of expansion based approaches. For Split mini-ImageNet and Split CIFAR-100 datasets, we set the memory size to 10,000 examples; we use 500 for other datasets. $^{*}$ and $^{**}$ over GMED methods indicate significant improvement over the counterparts without GMED with $p$-values less than $0.1$ and $0.05$ respectively in single-tailed paired t-tests. $^*$ and $^{**}$ over Previous SoTA results indicate significant improvement of the best performing GMED method over best performing baselines.
\arka{Maybe remove AGEM/GSS/BGD/HAL from this table.}
}
\label{tab:new_main_tab}

\centering
\scalebox{0.66}{\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Methods / Datasets} & \textbf{Task-free} &  \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Permuted\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rotated\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ CIFAR-10\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ CIFAR-100\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ mini-ImageNet\end{tabular}} \\ \midrule
Fine tuning & \ding{51}  & 18.80 $\pm$ 0.6  & 66.34 $\pm$ 2.6 & 41.24 $\pm$ 1.5 & 18.49 $\pm$ 0.2 & 3.06 $\pm$ 0.2 & 2.84 $\pm$ 0.4  \\
AGEM~\citep{chaudhry2018efficient} &\ding{51} & 29.02 $\pm$ 5.3 & 72.17 $\pm$ 1.5 & 50.77 $\pm$ 1.9 &   18.49 $\pm$ 0.6 & 2.40 $\pm$ 0.2 & 2.92 $\pm$ 0.3  \\
GSS-Greedy~\citep{Aljundi2019GradientBS} & \ding{51} & 84.16 $\pm$ 2.6 & 77.43 $\pm$ 1.4 & 73.66 $\pm$ 1.1  & 28.02 $\pm$ 1.3 & 19.53 $\pm$ 1.3 & 16.19 $\pm$ 0.7 \\
BGD~\citep{Zeno2018TaskAC} & \ding{51} & 13.54 $\pm$ 5.1 & 19.38 $\pm$ 3.0 & 77.94 $\pm$ 0.9 & 18.23 $\pm$ 0.5 & 3.11 $\pm$ 0.2 & 24.71 $\pm$ 0.8 \\
HAL~\citep{Chaudhry2020UsingHT} & \ding{55} & 77.92 $\pm$ 4.2 &  77.55 $\pm$ 4.2 & 78.48 $\pm$ 1.5 & 32.06 $\pm$ 1.5 & 21.11 $\pm$ 1.4 & 21.18 $\pm$ 2.1 \\
% \midrule
\midrule
%ER + GMED$_{\gamma=0.99}$   &    \ding{51}   &      82.60 $\pm$ 2.2                 &           79.15 $\pm$ 0.6              &        77.35 $\pm$ 1.3              &      34.10 $\pm$ 3.4           &   19.90 $\pm$ 1.5        &                          27.69 $\pm$ 0.7         \\
GEM~\citep{LopezPaz2017GradientEM} & \ding{55} & 87.18 $\pm$ 1.3 &  78.59 $\pm$ 1.0  & 78.40 $\pm$ 0.8 & 20.05 $\pm$ 1.4 &  8.75 $\pm$ 0.4 & 11.27 $\pm$ 3.4 \\
GEM + GMED   & \ding{55} &    87.64 $\pm$ 1.3                      &              78.67 $\pm$ 1.1                    &                      78.62 $\pm$    0.4           &      20.49 $\pm$ 1.5         &        8.72 $\pm$ 0.4            &   11.35 $\pm$ 0.3 \\
\midrule
ER~\citep{Robins1995CatastrophicFR} &  \ding{51}   & 80.96 $\pm$ 2.3                                                & 79.69 $\pm$ 1.0                                                   & 76.95 $\pm$ 1.7                                                  & 33.34 $\pm$ 1.5                               &    20.65 $\pm$ 1.3                 & 26.00 $\pm$ 1.0                                                        \\
ER + GMED    &   \ding{51}    & 82.68$^{**}$ $\pm$ 2.1                                           & 79.70 $\pm$ 1.1                                                   & 77.89$^{**}$ $\pm$ 0.9                                              & 36.21$^{**}$ $\pm$ 3.0                              &     20.87 $\pm$ 1.4        & 28.19$^{**}$ $\pm$ 0.8                                                    \\
\midrule
%MIR + GMED$_{\gamma=0.99}$    &   \ding{51}   &     86.76 $\pm$ 1.2                  &         79.76 $\pm$ 0.7               &         78.61 $\pm$ 0.6                &    35.78 $\pm$ 3.2      &    20.48 $\pm$ 1.7     &  27.70$^{**}$ $\pm$ 1.3   \\
MIR~\citep{Aljundi2019OnlineCL}  &  \ding{51}  & 84.88 $\pm$ 1.7                                                & 79.96 $\pm$ 1.3                                                   & 78.30 $\pm$ 1.0                                                  & 34.47 $\pm$ 2.0                          &    20.18 $\pm$ 1.7                      & 25.01 $\pm$ 1.3 \\
MIR + GMED  &   \ding{51}     & \textbf{87.86$^{**}$ $\pm$ 1.1}                                          & \textbf{80.11$^{**}$ $\pm$ 1.2}                                               & 79.16$^{**}$ $\pm$ 0.9                                           & 36.44$^{**}$ $\pm$ 1.1       &    \textbf{21.49$^{**}$ $\pm$ 0.6}                                        & 26.29$^{**}$ $\pm$ 1.2               \\
\midrule
ER$_{aug}$~\citep{Buzzega2020RethinkingER} & \ding{51}  & 79.91 $\pm$ 1.7                                                &         79.00 $\pm$ 0.8                               & 80.60 $\pm$ 1.3                                      & 47.34 $\pm$ 3.1                       &         18.66 $\pm$ 2.0                  &  31.36 $\pm$ 2.1      
\\
ER$_{aug}$ + GMED   & \ding{51} &  82.39$^{**}$ $\pm$ 2.1                                                &            79.08 $\pm$ 0.8                         & \textbf{80.66 $\pm$ 1.2}                                                 &   \textbf{48.34$^*$ $\pm$ 2.6}                  &         19.56 $\pm$ 1.3                  & \textbf{32.45$^{*}$ $\pm$ 1.2}   \\
% HAL + GMED & & & & & \\
\midrule
Previous SoTA &  - & 87.18 $\pm$ 1.3 &   79.96$^{**}$ $\pm$ 1.3  & 80.60 $\pm$ 1.3 & 47.34$^{**}$ $\pm$ 3.1 & 21.11 $\pm$ 1.4  & 31.36$^{*}$ $\pm$ 1.6   \\ 
iid online &  - & 85.99 $\pm$ 0.3 &   73.58 $\pm$ 1.5  & 81.30 $\pm$ 1.3 &  62.23 $\pm$ 1.5 & 18.13 $\pm$ 0.8  &  17.53 $\pm$ 1.6   \\
iid offline (upper bound) & - & 93.87 $\pm$ 0.5 &  87.40 $\pm$ 1.1  & 91.38 $\pm$ 0.7  & 76.36 $\pm$ 0.9 & 42.00 $\pm$ 0.9 & 37.46 $\pm$ 1.3 \\ 
% \textbf{ER + Random Edit} & 80.13 $\pm$ 2.9 & 78.85 $\pm$ 0.2 & 76.40 $\pm$ 1.7 & 34.72 $\pm$ 1.6 & 25.73 $\pm$ 2.0 \\
% \textbf{ER + Hindsight Edit} & 70.32 $\pm$ 3.9 & 79.23 $\pm$ 0.6 & 76.33 $\pm$ 1.1 & 33.08 $\pm$ 3.3 & 27.27 $\pm$ 1.7 \\
\bottomrule
\end{tabular}
}


\end{table*}

==> floats/merge_fuzzy_cndpm.tex <==
\begin{table*}
% \vspace{-0.2cm}
\centering
\begin{minipage}[t]{0.44\textwidth}
\centering
\caption{\small \textbf{Comparison with model-expansion-based approaches} under the same memory overhead as CN-DPM. The overhead is the size of the replay memory plus the extra model components (e.g. a generator or modules to solve individual tasks), shown in the equivalent number of memory examples (\#. Mem). $\dagger$ indicates quoted numbers are taken from the respective paper. \\}
\vspace{-0.2cm}
\scalebox{0.60}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Method}  & \multicolumn{2}{c}{\textbf{Split MNIST}} & \multicolumn{2}{c}{\textbf{Split CIFAR-10}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} \\ \midrule
\textbf{}        & Acc.        & \#. Mem          & Acc.       & \#. Mem  & Acc. &  \#. Mem   \\ \midrule
\textbf{CN-DPM}$^\dagger$  & 93.23       & 2,581               & 45.21      & 6,024     & 20.10 & 21,295  \\
\textbf{Prog. NN} & 89.46 & 9,755  & 49.68 & 6,604 & 19.17 & 31,766 \\
\textbf{CompCL} & 91.27 & 9,755 & 45.62 & 6,604 & 20.51 & 31,766 \\ 
\textbf{ER}      & 92.67       & 2,581                & 62.96      & 6,024    & 21.79 &   21,295    \\
\textbf{ER+GMED} & \best{94.16}       & 2,581             & \best{63.28 }     & 6,024     & \best{22.12} &   21,295    \\
\bottomrule 
\end{tabular}
}
\end{minipage}
\begin{minipage}[t]{0.53\textwidth}
\centering
\caption{\textbf{Performance of methods over data streams with fuzzy task boundaries}. In this setup, examples from the next tasks are introduced and gradually dominate the stream when half of the examples from the current task is visited. * indicates whether the improvement is significant ($p < 0.05$) \\
}

\label{tab:fuzzy_half}
\scalebox{0.50}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Methods / Datasets} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rotated\\ MNIST\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ CIFAR-10\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Split\\ mini-ImageNet\end{tabular}} \\ \midrule
\textbf{Vanilla}          &      21.53 $\pm$ 0.1                        &          42.58 $\pm$ 0.4                    &        20.69 $\pm$ 2.4       &                 3.05 $\pm$ 0.6                            \\
\textbf{AGEM}          &       25.30 $\pm$ 0.9                   &     52.21 $\pm$ 0.3            &     21.01 $\pm$ 0.2       &        3.88 $\pm$ 0.0                   \\
\textbf{ER}          &       79.74 $\pm$ 4.0                         &           76.45 $\pm$ 1.2                    &        37.15 $\pm$ 1.6        &                 26.47 $\pm$ 2.3                            \\
\textbf{MIR}         &              85.80 $\pm$ 1.9             &         77.04 $\pm$ 1.2                               &         38.70 $\pm$ 1.7           &            25.83 $\pm$ 1.5                                                \\
%\textbf{GSS-Greedy}          &                        &                     &          &                                          \\
\textbf{ER$_{aug}$}  &                  81.30 $\pm$ 2.0       &             \textbf{80.31 $\pm$ 0.9}                          &              47.97 $\pm$ 3.5          &           31.75 $\pm$ 1.0                     \\ \midrule
\textbf{ER + GMED}   &      82.73$^*$ $\pm$ 2.6                        &                  76.55 $\pm$ 1.0                    &        40.57$^*$ $\pm$ 1.7        &               28.20$^*$ $\pm$ 0.6                   \\                     

\textbf{MIR + GMED}  &                  \textbf{86.17 $\pm$ 1.7}       &             77.56$^*$ $\pm$ 1.1                          &        41.22$^*$ $\pm$ 1.1            &           26.86$^*$ $\pm$ 0.7                     \\ 

\textbf{ER$_{aug}$ + GMED}  &                  82.39$^*$ $\pm$ 3.7       &             80.30 $\pm$ 1.0                          &              \textbf{51.38$^*$ $\pm$ 2.2}             &           \textbf{31.83 $\pm$ 0.8}                     \\ \bottomrule



\end{tabular}
}

\end{minipage}
% \vspace{-0.7cm}
\end{table*}


==> floats/reg_abl.tex <==
% \begin{figure}[t]
% \vspace{-0.8cm}
%     \centering
%     %\subfloat[][Split MNIST \\(5 task)]{\includegraphics[width=0.2\linewidth]{figs/abl_split_mnist.pdf}}
%     %\subfloat[][Permuted MNIST\\(10 task)]{\includegraphics[width=0.2\linewidth]{figs/abl_permuted_mnist.pdf}}
%     \subfloat[][Rotated MNIST]{\includegraphics[width=0.40\linewidth]{figs/abl_rotated_mnist.pdf}}
%     %\subfloat[][Split CIFAR-10\\(5 task)]{\includegraphics[width=0.2\linewidth]{figs/abl_split_cifar.pdf}}
%     \subfloat[][Split mini-ImgNet]{\includegraphics[width=0.40\linewidth]{figs/abl_mini_imagenet.pdf}}
%     \vspace{-0.2cm}
%     \caption{Ablation study of the regularization term. We show the accuracy(\%) when we apply GMED without regularization (reg.) and with regularization. %For datasets that have more tasks, such as Rotated MNIST and Split mini-ImageNet, the improvements are more clear.
%     }
%     \label{fig:ablation_reg}
%     \vspace{-0.3cm}
% \end{figure}

% move to appendix
